Modified uncertainty relations from classical and quantum gravity

A good hundred years after the necessity for a quantum theory of gravity was acknowledged by Albert Einstein, the search for it continues to be an ongoing endeavour. Nevertheless, the field still evolves rapidly as manifested by the recent rise of quantum gravity phenomenology supported by an enormous surge in experimental precision. In particular, the minimum length paradigm ingrained in the program of generalized uncertainty principles (GUPs) is steadily growing in importance. The present thesis is aimed at establishing a link between modified uncertainty relations, derived from deformed canonical commutators, and curved spaces - specifically, GUPs and nontrivial momentum space as well as the related extended uncertainty principles (EUPs) and curved position space. In that vein, we derive a new kind of EUP relating the radius of geodesic balls, assumed to constrain the wave functions in the underlying Hilbert space, with the standard deviation of the momentum operator. This result is gradually generalized to relativistic particles in curved spacetime in accordance with the 3+1 decomposition. In a sense pursuing the inverse route, we find an explicit correspondence between theories yielding a GUP and quantum dynamics set on non-Euclidean momentum space. Quantitatively, the coordinate noncommutativity translates to momentum space curvature in the dual description, allowing for an analogous transfer of constraints from the literature. Finally, we find a formulation of quantum mechanics which proves consistent on the arbitrarily curved cotangent bundle. Along these lines, we show that the harmonic oscillator can not be used as a means to distinguish between curvature in position and momentum space, thereby providing an explicit instantiation of Born reciprocity in the context of curved spaces.

==> Main_and_Chapters/abstract2.tex <==
\section*{Summary of the Doctoral Thesis}
{University of Szczecin -- Institute of Physics -- Fabian Wagner, M. Sc.\\
	Title:} Modified uncertainty relations from classical and quantum gravity\\
{Supervisor:} prof. dr. hab. Mariusz D\k{a}browski\\
Auxiliary supervisor: dr. Husain Gohar\\
\noindent\makebox[\linewidth]{}

A good hundred years after the necessity for a quantum theory of gravity was acknowledged by Albert Einstein, the search for it continues to be an ongoing endeavour. Nevertheless, the field still evolves rapidly as manifested by the recent rise of quantum gravity phenomenology supported by an enormous surge in experimental precision. In particular, the minimum length paradigm ingrained in the program of generalized uncertainty principles (GUPs) is steadily growing in importance. 

The present thesis is aimed at establishing a link between modified uncertainty relations, derived from deformed canonical commutators, and curved spaces - specifically, GUPs and nontrivial momentum space as well as the related extended uncertainty principles (EUPs) and curved position space. In that vein, we derive a new kind of EUP relating the radius of geodesic balls, assumed to constrain the wave functions in the underlying Hilbert space,  with the standard deviation of the momentum operator, suitably made compatible with the curved spatial background. This result is gradually generalized to relativistic particles in curved spacetime in accordance with the 3+1 decomposition, thereby relating semiclassical gravity with the EUP. 

The corresponding corrections to the relation in flat space depend on the Ricci scalar of the effective spatial metric, the lapse function and the shift vector, as well as covariant derivatives thereof. The ensuing inequality is evaluated in Rindler, de Sitter and Schwarzschild backgrounds, at lowest approximation leading to identical effects, as well as to rotating geometries like Kerr black holes and their analogues in higher-order theories of gravity. 

In a sense pursuing the inverse route, we find an explicit correspondence between theories yielding a GUP, possibly including a noncommutative geometry, and quantum dynamics set on non-Euclidean momentum space. Quantitatively, the coordinate noncommutativity translates to momentum space curvature in the dual description, allowing for an analogous transfer of constraints from the literature. However, a commutative geometry does not imply trivial dynamics; the corresponding types of GUP lead to a flat momentum space, described in terms of a nontrivial basis, permitting the import of further bounds. 

Finally, we find a formulation of quantum mechanics which proves consistent on the arbitrarily curved cotangent bundle. Along these lines, we show that the harmonic oscillator can, given a suitable choice of operator ordering, not be used as a means to distinguish between curvature in position and momentum space, thereby providing an explicit instantiation of Born reciprocity in the context of curved spaces.\\
\noindent\makebox[\linewidth]{}
Date, signature:

==> Main_and_Chapters/declaration.tex <==
% ******************************* Thesis Declaration ***************************
\section*{O\'swiadczenie doktoranta}
\markright{O\'swiadczenie doktoranta}

%\begin{declaration}

O\'swiadczam, \.ze moja praca pt.: {\bfseries Modified uncertainty relations from classical and quantum gravity}
\begin{enumerate}[a]
	\item zosta{\l}a napisana przeze mnie samodzielnie,
	\item nie narusza praw autorskich w rozumieniu ustawy z dnia 14 lutego 1994 roku o prawie autorskim i prawach pokrewnych (Dz.U. 2019 r. poz. 1231) oraz d\'obr osobistych chronionych prawem,
	\item nie zawiera danych i informacji, kt\'o re uzyskałem w sposób niedozwolony,
	\item nie była podstawą nadania tytu{\l}u naukowego lub zawodowego ani mnie ani innej osobie.
\end{enumerate}
Ponadto o\'swiadczam, \.ze tre\'s\'c pracy przedstawionej przeze mnie do obrony, zawarta na przekazanym no\'sniku elektronicznym jest identyczna z jej wersją drukowan\k{a}.

 
\vspace*{4em}\noindent
\hfill%
\begin{tabular}[t]{c}
  \rule{10em}{0.4pt}\\ Miasto, data
\end{tabular}%
\hfill%
\begin{tabular}[t]{c}
  \rule{10em}{0.4pt}\\ Fabian Wagner
\end{tabular}%
\hfill\strut

\vspace*{4em}\noindent
\begingroup
\renewcommand{\cleardoublepage}{}
\renewcommand{\clearpage}{}
\section*{O\'swiadczenie}
\endgroup

Wyra\.zam zgod\k{e} na udostępnienie mojej pracy doktorskiej pt.: {\bfseries Modified uncertainty relations from classical and quantum gravity}.

\vspace*{4em}\noindent
\hfill%
\begin{tabular}[t]{c}
	\rule{10em}{0.4pt}\\ Miasto, data
\end{tabular}%
\hfill%
\begin{tabular}[t]{c}
	\rule{10em}{0.4pt}\\ Fabian Wagner
\end{tabular}%
\hfill\strut

\vspace*{4em}\noindent
\begingroup
\renewcommand{\cleardoublepage}{}
\renewcommand{\clearpage}{}
\section*{O\'swiadczenie}
\endgroup

Akceptuję ostateczną wersję pracy.

\vspace*{4em}\noindent
\hfill%
\begin{tabular}[t]{c}
	\rule{10em}{0.4pt}\\ Miasto, data
\end{tabular}%
\hfill%
\begin{tabular}[t]{c}
	\rule{10em}{0.4pt}\\ prof. Mariusz D\k{a}browski
\end{tabular}%
\hfill\strut

% Author and date will be inserted automatically from thesis.tex \author \degreedate

%\end{declaration}



==> Main_and_Chapters/streszczenie.tex <==
\section*{Streszczenie rozprawy doktorskiej}

Uniwersytet Szczeci\'nski -- Institut Fizyki -- mgr. Fabian Wagner\\
Tytu{\l}: Modified uncertainty relations from classical and quantum gravity\\
Promotor: prof. dr. hab. Mariusz D\k{a}browski\\
Promotor pomocniczy: dr. Husain Gohar\\
\noindent\makebox[\linewidth]{}

Chocia\.z min\k{e}{\l}o ponad sto lat od momentu, w kt\'orym  Albert Einstein uzna{\l}  konieczno\'s\'c stworzenia kwantowej teorii grawitacji, to poszukiwanie jej ostatecznego kszta{\l}tu wci\k{a}\.z pozostaje wyzwaniem. Dziedzina ta nadal dynamicznie si\k{e} rozwija czego dowodem jest ostatni wzrost bada\'n w zakresie fenomenologii kwantowej grawitacji wspierany przez niesamowit\k{a} popraw\k{e} dok{\l}adno\'sci eksperyment\'ow w mechanice kwantowej. W szczeg\'olno\'sci, coraz wi\k{e}ksz\k{a} rol\k{e} odgrywa postulat istnienia minimalnej d{\l}ugo\'sci fizyce maj\k{a}cy \'scis{\l}y zwi\k{a}zek z og\'olnion\k{a} zasad\k{a} nieoznaczono\'sci (UZN) Heisenberga. 

Niniejsza rozprawa ma na celu ustalenie zwi\k{a}zk\'ow pomi\k{e}dzy zmodyfikowanymi zasadami nieoznaczono\'sci wywodz\k{a}cymi si\k{e} ze zdeformowanych komutator\'ow kanonicznych a zakrzywionymi przestrzeniami - w szczeg\'olno\'sci z UZN i nietrywialn\k{a} przestrzeni\k{a} p\k{e}du - a tak\.ze zwi\k{a}zanymi z nimi rozszerzonymi zasadami nieoznaczono\'sci (RZN) i zakrzywion\k{a} przestrzeni\k{a} po{\l}o\.zenia. W tym duchu wprowadzamy nowy rodzaj RZN, wi\k{a}\.z\k{a}cy promienie kul geodezyjnych stosowanych do ograniczania funkcji falowych z przestrzeni Hilberta, z odchyleniem standardowym operatora p\k{e}du odpowiednio dostosowanego do zakrzywionej przestrzeni t{\l}a. Wynik ten stopniowo jest uog\'olniany na cz\k{a}stki relatywistyczne w zakrzywionej czasoprzestrzeni w formali\'zmie ADM rozwarstwienia 3+1, wi\k{a}\.z\k{a}c tym samym p\'o{\l}klasyczn\k{a} grawitacj\k{e} z RZN. 


Odpowiednie poprawki do RZN w p\l askiej przestrzeni zale\.z\k{a} od skalara Ricciego efektywnej metryki przestrzennej, funkcji poklatkowej (lapse) i wektora przesuni\k{e}cia (shift), a tak\.ze od ich pochodnych kowariantnych. Wynikaj\k{a}ca z tego nier\'owno\'s\'c RZN jest wyliczana w najni\.zszym rz\k{e}dzie rachunku zaburze\'n dla czasoprzestrzeni Rindlera, de Sittera i Schwarzschilda prowadz\k{a}c do podobnych jako\'sciowo rezultat\'ow, oraz dla rotuj\k{a}cych czasoprzestrzeni czarnych dziur Kerra i ich odpowiednik\'ow w teoriach grawitacji wy\.zszego rz\k{e}du. 

Stosuj\k{a}c w pewnym sensie podej\'scie odwrotne, znajdujemy jawn\k{a} korespondencj\k{e} pomi\k{e}dzy teoriami prowadz\k{a}cymi do UZN, prawdopodobnie obejmuj\k{a}cymi geometri\k{e} nieprzemienn\k{a}, a dynamik\k{a} kwantow\k{a} opart\k{a} na nieeuklidesowej przestrzeni p\k{e}du. Ilo\'sciowo, nieprzemienno\'s\'c 
wsp\'o{\l}rz\k{e}dnych przek\l ada si\k{e} na krzywizn\k{e} przestrzeni p\k{e}du w opisie dualnym, co pozwala na analogiczne przeniesienie znanych z literatury ogranicze\'n dla UZN, na ograniczenia dla przestrzeni p\k{e}du. 

Ciekawe jest, \.ze geometria przemienna nie implikuje trywialnej dynamiki - odpowiadaj\k{a}ce jej typy UZN prowadz\k{a} do p\l askiej przestrzeni p\k{e}d\'ow, opisanej w kategoriach nietrywialnej bazy, pozwalaj\k{a}cej na dalszy import ogranicze\'n. W ko\'ncu znajdujemy sformu\l owanie mechaniki kwantowej, kt\'ore okazuje si\k{e} sp\'ojne w przypadku dowolnie zakrzywionej wi\k{a}zki kostycznej. W tym sformu{\l}owaniu pokazujemy, \.ze przy w{\l}a\'sciwym doborze uporz\k{a}dkowania operator\'ow, oscylator harmoniczny nie mo\.ze by\'c u\.zyty do rozr\'o\.znienia krzywizny w przestrzeni po{\l}o\.zenia i w przestrzeni p\k{e}du, co zapewnia klarowny przyk{\l}ad dualno\'sci Borna w kontek\'scie zakrzywionych przestrzeni.\\
\noindent\makebox[\linewidth]{}
Data, podpis:

==> fig/mindmap.tex <==
\begin{tikzpicture}[ every annotation/.style = {draw,
                     fill = white, font = \Large}]
  \path[mindmap,concept color=black,text=white,
    every node/.style={concept,circular drop shadow},
    root/.style    = {concept color=black,
      font=\large\bfseries,text width=10em},
    level 1 concept/.append style={font=\Large\bfseries,
      sibling angle=100,text width=7.7em,
    level distance=15em,inner sep=0pt},
    level 2 concept/.append style={level distance=9em,
      sibling angle=50},
  ]
  node[root] {Quantum Gravity} [clockwise from=-40]
    child[concept color=myblue] {
      node {Covariant} [clockwise from=110]
        child { node[concept] (hl) {Hor\v{r}ava-Lifshitz gravity}} 
        child { node[concept] (strings) {String theory}} 
        child{ node (adscft) {AdS/ CFT}}
        child { node (CDT) {Causal \mbox{Dynamical} Triangulations} }
        child {node (AS) {Asymp\-totic Safety}}
        child {node (eucl) {Euclidean Quantum Gravity}}
        child {node (sf) {Spinfoam models}}
    }
    child[concept color=green!40!black] {
      node[concept] {Canonical}
        [clockwise from=-30]
        child { node[concept] (LQG)
        {Loop Quantum Gravity}}
      child { node[concept] (WdW)
        {Quantum Geometro\-dynamics}[clockwise from=-10]
        child[concept color=mix,scale=1.6] {node[concept,scale=1.5] (QC) {Quantum Cosmology}}}
      child { node[concept] (CaPert)
        {Pertur\-bative Quantum Gravity}}
    };
\newcommand{\redtoblue}{to[circle connection bar switch color=from (mix) to (myblue)]}
\newcommand{\redtogreen}{to[circle connection bar switch color=from (mix) to (green!40!black)]}
\newcommand{\bluetogreen}{to[circle connection bar switch color=from (myblue) to (green!40!black)]}
\newcommand{\bluetoblue}{to[circle connection bar switch color=from (myblue) to (myblue)]}
\begin{pgfonlayer}{background}
    %\draw [circle connection bar ]
    \path (QC) \redtoblue (eucl);
    \path (QC) \redtoblue (sf);
    \path (QC) \redtogreen (LQG);
    \path (sf) \bluetogreen (LQG);
    \path (eucl) \bluetoblue (AS);
    \path (CDT) \bluetoblue (AS);
    \path (adscft) \bluetoblue (strings);
\end{pgfonlayer}    
\end{tikzpicture}

==> fig/mindmap2.tex <==
\begin{tikzpicture}[ every annotation/.style = {draw,
                     fill = white, font = \Large}]
  \node[extra concept,scale=8.4,color=burgundy,text=white,font=\fontsize{3}{12}\bfseries] at ($(0,-2.6)$){} ;
  \node[text=white,font=\Huge\bfseries,align=center] at (0,3.3) {Curved\\ Momentum Space};
  \path[mindmap,concept color=black,text=white,
    every node/.style={concept,circular drop shadow},
    root/.style    = {concept color=black,
      font=\Large\bfseries,text width=10em},
    level 1 concept/.append style={font=\large\bfseries,
      sibling angle=50,text width=7.7em,
    level distance=15em,inner sep=0pt},
    level 2 concept/.append style={level distance=9em,
      sibling angle=50},
  ]
  node[root] (ML){Minimum length} [clockwise from=-40]
    child[concept color=myblue] {
      node (DSR){Deformed Special Relativity} [clockwise from=110]
    }
    child[concept color=mix,scale=1.3]{node (GUP)
        {Generalized \mbox{Uncertainty} Principle}}
    child[concept color=green!40!black] {
      node[concept] (LIV){Lorentz Invariance Violation}
        [clockwise from=-30]
    };
\newcommand{\mixtoblue}{to[circle connection bar switch color=from (mix) to (myblue)]}
\newcommand{\greentomix}{to[circle connection bar switch color=from (green!40!black) to (mix)]}
\begin{pgfonlayer}{foreground}
    %\draw [circle connection bar ]
    \path (GUP) \mixtoblue (DSR);
    \path (LIV) \greentomix (GUP);
\end{pgfonlayer}    
\end{tikzpicture}


